Better Algorithms for Hybrid Circuit and Packet Switching in Data Centers

Hybrid circuit and packet switching for data center networking (DCN) has received considerable research attention recently. A hybrid-switched DCN employs a much faster circuit switch that is reconfigurable with a nontrivial cost, and a much slower packet switch that is reconfigurable with no cost, to interconnect its racks of servers. The research problem is, given a traffic demand matrix (between the racks), how to compute a good circuit switch configuration schedule so that the vast majority of the traffic demand is removed by the circuit switch, leaving a remaining demand matrix that contains only small elements for the packet switch to handle. In this paper, we propose two new hybrid switch scheduling algorithms under two different scheduling constraints. Our first algorithm, called 2-hop Eclipse, strikes a much better tradeoff between the resulting performance (of the hybrid switch) and the computational complexity (of the algorithm) than the state of the art solution Eclipse/Eclipse++. Our second algorithm, called BFF (best first fit), is the first hybrid switching solution that exploits the potential partial reconfiguration capability of the circuit switch for performance gains.

==> libs/autoref_custom.tex <==
% use "autoref" the way I want
%   autoref is nice because the text or brackets of a ref are part of link
%   see http://tex.stackexchange.com/questions/36575/autorefs-inserted-text-has-not-the-correct-case
%       http://en.wikibooks.org/wiki/LaTeX/Labels_and_Cross-referencing
%       http://www.tug.org/applications/hyperref/manual.html#TBL-23

%% define autoref name for sections
% \ifx\sectionautorefname\defined
\def\sectionautorefname{\S\!\!}
\def\subsectionautorefname{\S\!\!}
\def\subsubsectionautorefname{\S\!\!}
% \fi
% from http://tex.stackexchange.com/questions/52410/how-to-use-the-command-autoref-to-implement-the-same-effect-when-use-the-comman
% \ifx\equationautorefname~#1\undefined
\def\equationautorefname~#1\null{%
  (#1)\null
}
% \fi
